ExaGeoStat: A High Performance Unified Software for Geostatistics on Manycore Systems

We present ExaGeoStat, a high performance framework for geospatial statistics in climate and environment modeling. In contrast to simulation based on partial differential equations derived from first-principles modeling, ExaGeoStat employs a statistical model based on the evaluation of the Gaussian log-likelihood function, which operates on a large dense covariance matrix. Generated by the parametrizable Matern covariance function, the resulting matrix is symmetric and positive definite. The computational tasks involved during the evaluation of the Gaussian log-likelihood function become daunting as the number n of geographical locations grows, as O(n2) storage and O(n3) operations are required. While many approximation methods have been devised from the side of statistical modeling to ameliorate these polynomial complexities, we are interested here in the complementary approach of evaluating the exact algebraic result by exploiting advances in solution algorithms and many-core computer architectures. Using state-of-the-art high performance dense linear algebra libraries associated with various leading edge parallel architectures (Intel KNLs, NVIDIA GPUs, and distributed-memory systems), ExaGeoStat raises the game for statistical applications from climate and environmental science. ExaGeoStat provides a reference evaluation of statistical parameters, with which to assess the validity of the various approaches based on approximation. The framework takes a first step in the merger of large-scale data analytics and extreme computing for geospatial statistical applications, to be followed by additional complexity reducing improvements from the solver side that can be implemented under the same interface. Thus, a single uncompromised statistical model can ultimately be executed in a wide variety of emerging exascale environments.

==> Makefile <==
# LaTeX -*-Makefile-*-
#
# $HEADER$
# 

# MAIN_TEX: In order to build your document, fill in the MAIN_TEX
# macro with the name of your main .tex file -- the one that you
# invoke LaTeX on.

MAIN_TEX	= exageostat-1file.tex

# OTHER_SRC_FILES: Put in the names of all the other .tex files that
# this document depends on in the OTHER_SRC_FILES macro.  This is
# ensure that whenever one of the "other" files changes, "make" will
# rebuild your paper.

#OTHER_SRC_FILES	= intro.tex summary.tex \
#                  abstract.tex perf.tex rw.tex \
#		  pb.tex impl.tex ack.tex \
#		  geospat.tex contrib.tex



# BibTeX sources.  The bibliography will automatically be re-generated
# if these files change.

BIBTEX_SOURCES = references.bib

# xfig figures.  Will be converted to .eps and .pdf as necessary.

FIG_FILES	=

# Files that alredy exist as .png.  Will be converted to .eps and .pdf
# as necessary.

PNG_FILES	= 

# Files that alredy exist as .eps.  Will be converted to .pdf as
# necessary.

EPS_FILES	= 


# Required commands and options

LATEX		= latex
PDFLATEX	= pdflatex
DVIPS		= dvips
MAKEINDEX	= makeindex
BIBTEX		= bibtex
FIG2DEV		= fig2dev
PNGTOPNM	= pngtopnm
PNMTOPS		= pnmtops
EPS2PDF		= epstopdf
PS2PDF          = ps2pdf
PS2PDF_OPTIONS  = -sPaperSize=letter -dAutoFilterGrayImages=false \
		-dGrayDownSample=false -sGrayImageFilter=LZWEncode \
		-dAutoFilterColorImages=false -sColorImageFilter=LZWEncode \
		-dColorDownSample=false -dEmbedAllFonts=true \
		-dSubsetFonts=true
DISTILL         = distill
DISTILL_OPTIONS = -v -pagesize 612 792 pts -encodegray on -graycompr lzw \
		-graydownsample off -grayacs off -graydepth 8 \
		-subsetfonts on -embedallfonts on -pairs
PSNUP           = psnup

#########################################################################
#
# You should not need to edit below this line
#
#########################################################################

.SUFFIXES:	.tex .dvi .ps .pdf .fig .eps .png

MAIN_DVI	= $(MAIN_TEX:.tex=.dvi)
MAIN_PS		= $(MAIN_TEX:.tex=.ps)
MAIN_PDF	= $(MAIN_TEX:.tex=.pdf)
MAIN_BBL	= $(MAIN_TEX:.tex=.bbl)
MAIN_BASENAME	= $(MAIN_TEX:.tex=)
EPS_PNG_FILES	= $(PNG_FILES:.png=.eps)
EPS_FIG_FILES	= $(FIG_FILES:.fig=.eps)
PDF_FIG_FILES	= $(FIG_FILES:.fig=.pdf)
PDF_EPS_FILES	= $(EPS_FILES:.eps=.pdf)

#
# Some common target names
# Note that the default target is "ps"
#

pdf: $(MAIN_PDF)
ps: $(MAIN_PS) 

#
# Make the dependencies so that things build when they need to
#

$(MAIN_PS): $(MAIN_DVI)
$(MAIN_DVI): $(MAIN_TEX) $(CITE_TEX) $(OTHER_SRC_FILES) $(EPS_FIG_FILES) $(EPS_FILES) $(MAIN_BBL)
$(MAIN_PDF): $(MAIN_TEX) $(CITE_TEX) $(OTHER_SRC_FILES) $(PDF_FIG_FILES) $(PNG_FILES) $(MAIN_BBL) $(PDF_EPS_FILES)

#
# Search strings
#

REFERENCES = "(There were undefined references|Rerun to get (cross-references|the bars) right|No file *[aux|toc|lof|lot])"
NEEDINDEX = "Writing index file"
RERUNBIB = "No file.*\.bbl|LaTeX Warning: Citation|LaTeX Warning: Label\(s\) may"

#
# General rules
#

.fig.eps:
	$(FIG2DEV) -L eps $< $@

.fig.pdf:
	$(FIG2DEV) -L pdf $< $@

.eps.pdf:
	@if ( `which $(DISTILL) > /dev/null 2>&1` ); then \
		cmd="$(DISTILL) $(DISTILL_OPTIONS) $*.eps $*.pdf" ; \
                echo $$cmd ; \
                eval $$cmd ;\
	elif ( which $(EPS2PDF) > /dev/null 2>&1 ); then \
		cmd="$(EPS2PDF) $(EPS2PDF_OPTIONS) $*.eps " ; \
                echo $$cmd ; \
                eval $$cmd ;\
	elif ( which $(PS2PDF) > /dev/null 2>&1 ); then \
		cmd="$(PS2PDF) $(PS2PDF_OPTIONS) $*.eps $*.pdf" ; \
                echo $$cmd ; \
                eval $$cmd ;\
	else \
		echo "Cannot find ps to pdf converter :-("; \
	fi

.png.eps:
	$(PNGTOPNM) $< | $(PNMTOPS) -noturn > $*.eps

# Only run bibtex if latex has already been run (i.e., if there is
# already a .aux file).  If .aux file does not exist, then bibtex will
# be run during the .tex.dvi / .tex.pdf rules.  We don't run latex
# here to generate the .aux file because a) we don't know whether to
# run latex or pdflatex, and b) the dependencies are wrong for
# pdflatex because we may need to generate some pdf images first.

$(MAIN_BBL): $(BIBTEX_SOURCES)
	@if (test -f $(MAIN_BASENAME).aux); then \
		echo "### Running BibTex"; \
		$(BIBTEX) $(MAIN_BASENAME); \
	fi

# Macro to handle when running "latex" fails -- ensure to kill the
# .aux and .dvi files so that the next time we run "make", the
# .tex.dvi rule fires, not the .bbl or .dvi.ps rule.

DVI_FAIL = ($(RM) $(MAIN_BASENAME).aux $(MAIN_BASENAME).dvi && false)

# Main workhorse for .tex -> .dvi.  Run latex, makeindex, and bibtex
# as necessary.

.tex.dvi:
	@echo "### Running LaTeX (1)"
	$(LATEX) $* || $(DVI_FAIL)
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running LaTeX to fix references (2)"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(NEEDINDEX) $*.log >/dev/null); then \
		echo "### Running makeindex to generate index"; \
		$(MAKEINDEX) $*; \
		echo "### Running LaTeX after generating index"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(RERUNBIB) $*.log >/dev/null); then \
		echo "### Running BibTex because references changed"; \
		$(BIBTEX) $(MAIN_BASENAME); \
		echo "### Running LaTeX after generating bibtex"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running LaTeX to fix references (3)"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running LaTeX to fix references (4)"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi

.dvi.ps:
	$(DVIPS) -o $*.ps $*

# Macro to handle when running "latex" fails -- ensure to kill the
# .aux file so that the next time we run "make", the .tex.pdf rule
# fires, not the .bbl rule.

PDF_FAIL = ($(RM) $(MAIN_BASENAME).aux && false)

# Main workhorse for .tex -> .pdf.  Run latex, makeindex, and bibtex
# as necessary.  Essentially the same as .tex.dvi, except
# s/latex/pdflatex/ig.

.tex.pdf:
	@echo "### Running pdfLaTeX (1)"
	$(PDFLATEX) $* || $(PDF_FAIL)
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running pdfLaTeX to fix references (2)"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(NEEDINDEX) $*.log >/dev/null); then \
		echo "### Running makeindex to generate index"; \
		$(MAKEINDEX) $*; \
		echo "### Running pdfLaTeX after generating index"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(RERUNBIB) $*.log >/dev/null); then \
		echo "### Running BibTex because references changed"; \
		$(BIBTEX) $(MAIN_BASENAME); \
		echo "### Running pdfLaTeX after generating bibtex"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running pdfLaTeX to fix references (3)"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running pdfLaTeX to fix references (4)"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi

#
# graphs
#

Graph: graphs
graph: graphs
graphs:
	(cd results/la-myri; ./geplot)

#
# Just for fun
#

RUN_PSNUP = $(PSNUP) -d -b2 -m10 -pletter
1: $(MAIN_PS)
	num_pages="`psnup -1 $(MAIN_PS) bogus.ps 2>&1 | grep Wrote | cut -dW -f2- | awk '{ print $$2 }'`"; \
	$(RM) bogus.ps; \
	$(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	if test "$$?" != "0"; then \
	  num_pages="`expr $$num_pages + 1`"; \
	  $(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	fi; \
	if test "$$?" != "0"; then \
	  num_pages="`expr $$num_pages + 1`"; \
	  $(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	fi; \
	if test "$$?" != "0"; then \
	  num_pages="`expr $$num_pages + 1`"; \
	  $(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	fi
	$(RUN_PS2PDF) one-page.ps
	$(RM) one-page.ps

#
# Standard targets
#

clean:
	$(RM) *~ *.bak *%
	$(RM) *.aux *.dvi *.blg *.toc *.bbl *.lof *.lot \
		*.idx *.ilg *.int *.out */*.aux *.synctex.gz \
		$(EPS_PNG_FILES) $(EPS_FIG_FILES) $(PDF_FIG_FILES) \
		 $(PDF_EPS_FILES)

distclean: clean
	$(RM) $(MAIN_PS) $(MAIN_DVI) $(MAIN_PDF)

exageostat-1file-diff.pdf: exageostat-1file-orig.tex exageostat-1file.tex
	#make -C figures
	latexdiff exageostat-1file-orig.tex exageostat-1file.tex > exageostat-1file-diff.tex
	pdflatex -d exageostat-1file-diff

